A fast algorithm for computing Bell polynomials based on index break-downs using prime factorization

By establishing an interesting connection between ordinary Bell polynomials and rational convolution powers, some composition and inverse relations of Bell polynomials as well as explicit expressions for convolution roots of sequences are obtained. Based on these results, a new method is proposed for calculation of partial Bell polynomials based on prime factorization. It is shown that this method is more efficient than the conventional recurrence procedure for computing Bell polynomials in most cases, requiring far less arithmetic operations. A detailed analysis of the computation complexity is provided, followed by some numerical evaluations.

==> Bib.tex <==
@inproceedings{liu2008sufficient,
  title={Sufficient conditions for non-negative impulse response of arbitrary-order systems},
  author={Liu, Yuzhe and Bauer, Peter H},
  booktitle={APCCAS 2008-2008 IEEE Asia Pacific Conference on Circuits and Systems},
  pages={1410--1413},
  year={2008},
  organization={IEEE}
}
@inproceedings{liu2009pole,
  title={On pole-zero patterns of non-negative impulse response discrete-time systems with complex poles and zeros},
  author={Liu, Y and Bauer, Peter H},
  booktitle={2009 17th Mediterranean Conference on Control and Automation},
  pages={1102--1107},
  year={2009},
  organization={IEEE}
}
@inproceedings{malik2009transient,
  title={On the transient control of linear time invariant systems},
  author={Malik, Waqar A and Darbha, Swaroop and Bhattacharyya, SP},
  booktitle={2009 American Control Conference},
  pages={3142--3147},
  year={2009},
  organization={IEEE}
}
@inproceedings{mohsenizadeh2011synthesis,
  title={Synthesis of Digital PID Controllers for Discrete-time Systems with Guaranteed Non-overshooting Transient Response},
  author={Mohsenizadeh, Navid and Darbha, Swaroop and Bhattacharyya, Shankar P},
  booktitle={ASME 2011 Dynamic Systems and Control Conference and Bath/ASME Symposium on Fluid Power and Motion Control},
  pages={473--478},
  year={2011},
  organization={American Society of Mechanical Engineers}
}
@article{schmid2010unified,
  title={A unified method for the design of nonovershooting linear multivariable state-feedback tracking controllers},
  author={Schmid, Robert and Ntogramatzidis, Lorenzo},
  journal={Automatica},
  volume={46},
  number={2},
  pages={312--321},
  year={2010},
  publisher={Elsevier}
}
@article{schmid2012design,
  title={The design of nonovershooting and nonundershooting multivariable state feedback tracking controllers},
  author={Schmid, Robert and Ntogramatzidis, Lorenzo},
  journal={Systems \& Control Letters},
  volume={61},
  number={6},
  pages={714--722},
  year={2012},
  publisher={Elsevier}
}
@article{garone2015linear,
  title={Linear matrix inequalities for globally monotonic tracking control},
  author={Garone, Emanuele and Ntogramatzidis, Lorenzo},
  journal={Automatica},
  volume={61},
  pages={173--177},
  year={2015},
  publisher={Elsevier}
}
@article{Taghavian,
  title={On convolution powers, roots and inverses},
  author={Taghavian, Hamed},
  journal={},
  volume={},
  pages={},
  year={2017},
  publisher={zenodo}
}
@book{Dorf,
  title={The Engineering Handbook},
  author={Dorf, Richard C.},
  journal={},
  volume={},
  pages={},
  year={2018},
  publisher={}
}

@article{abu2014estimates,
  title={Estimates for the numerical radius and the spectral radius of the Frobenius companion matrix and bounds for the zeros of polynomials},
  author={Abu-Omar, Amer and Kittaneh, Fuad and others},
  journal={Ann. Funct. Anal},
  volume={5},
  number={1},
  pages={56--62},
  year={2014}
}
@article{chen1996combinatorial,
  title={The combinatorial power of the companion matrix},
  author={Chen, William YC and Louck, James D},
  journal={Linear Algebra and Its Applications},
  volume={232},
  pages={261--278},
  year={1996},
  publisher={Elsevier}
}












